Model-less Is the Best Model: Generating Pure Code Implementations to Replace On-Device DL Models

Recent studies show that deployed deep learning (DL) models such as those of Tensor Flow Lite (TFLite) can be easily extracted from real-world applications and devices by attackers to generate many kinds of attacks like adversarial attacks. Although securing deployed on-device DL models has gained increasing attention, no existing methods can fully prevent the aforementioned threats. Traditional software protection techniques have been widely explored, if on-device models can be implemented using pure code, such as C++, it will open the possibility of reusing existing software protection techniques. However, due to the complexity of DL models, there is no automatic method that can translate the DL models to pure code. To fill this gap, we propose a novel method, CustomDLCoder, to automatically extract the on-device model information and synthesize a customized executable program for a wide range of DL models. CustomDLCoder first parses the DL model, extracts its backend computing units, configures the computing units to a graph, and then generates customized code to implement and deploy the ML solution without explicit model representation. The synthesized program hides model information for DL deployment environments since it does not need to retain explicit model representation, preventing many attacks on the DL model. In addition, it improves ML performance because the customized code removes model parsing and preprocessing steps and only retains the data computing process. Our experimental results show that CustomDLCoder improves model security by disabling on-device model sniffing. Compared with the original on-device platform (i.e., TFLite), our method can accelerate model inference by 21.8% and 24.3% on x86-64 and ARM64 platforms, respectively. Most importantly, it can significantly reduce memory consumption by 68.8% and 36.0% on x86-64 and ARM64 platforms, respectively.

==> 3_Preliminary.tex <==
\section{Problem Analysis: Identifying Model Files}
% As we introduced in the last section, we need to convert the DL model to pure code implementations. However, it has two main problems: 1) the first problem is how the extract the corresponding code unit for each operator used in the DL model. Because the DL library usually

% \lili{We need to make it clear why we this preliminary study is needed.}
Before we present our proposed solution we show the potential risks of existing model deployment strategies in the interaction between the DL library and model files.
We investigate DL models on Android applications and analyze how attackers can identify such DL components in deployment environments. 

\label{sec::pre_file}
DL model files contain the DL model architecture and weights information. In the TFLite library, the model file is \texttt{.tflite} file. In TVM, 
it uses a graph file and a parameter file to store the information. These files are necessary for the on-device library or compiled AI programs to run on edge devices. Other DL compilers like Apple Core ML also apply
the file formats \texttt{.espresso.net} and \texttt{.espresso.weights} to store computational graphs and weights. 
% The process of model inference is shown in Figure~\ref{fig:on_device_inference}. In TFLite, the TFLite library will first load the model files, and then build a computational graph. The computational graph defines the data flow for model inference. Next, it loads the weights into the program. Finally, the TFLite library will compute the output according to the computational graph and given weights. AI compilers like TVM have a similar process at runtime unless they use low-level intermediate representation (IR) instead of high-level representation. 

% \begin{figure}[t]
%   \begin{center}
%     \includegraphics[width=0.92\linewidth]{figs/on_device_inference.pdf}
%   \end{center}
%   \vspace{-1em}
%   \caption{The typical process of model inference. TFLite and TVM use high-level and low-level intermediate representation (IR) to define the model information, respectively. }
%   \label{fig:on_device_inference}
% \end{figure}

Following ~\cite{xu2019first}, we investigate how to use keywords to identify a DL model in Android apps. The name of the TFLite model file ends with `\texttt{.tflite}' or `\texttt{.lite}', and the source codes of apps will call TensorFlow-related APIs. The cases for TVM are similar, the model information will be stored in `\texttt{graph.json}' (computational graph) and `\texttt{.params}' (weights). Inferences can be performed using those libraries by loading them into a shared library `\texttt{libtvm\_runtime.so}' \footnote{\href{https://tvm.apache.org/docs/arch/model\_library\_format.html}{https://tvm.apache.org/docs/arch/model\_library\_format.html}}. To simplify the analysis but without loss of generality, we use the TFLite model as the example.
% \vspace{-1em}

\paragraph{\textbf{Study Process}}
To identify DL components in real apps, we use the AndroZoo~\cite{allix2016androzoo} dataset to first collect a set of real-world Android apps.
%AndroZoo is by far the largest app set well maintained by researchers and has been widely leveraged by researchers to support various Android-related studies.
 AndroZoo contains over 23 million Android apps. It is extremely time-consuming for us to download and scan all of them to locate TFLite models.
For the sake of simplicity, we only focus on a subset of 173,905 apps collected from the official Google Play market to fulfill our study. After downloading those apps, we first simply use the `\texttt{org.tensorflow}' keyword to search the apps that may use TensorFlow APIs. All of these apps are regarded as candidates to extract TFLite models. Then, we use `\texttt{.tflite}' and `\texttt{.lite}' keywords to identify the app packages with DL models. 

% \begin{table}[t]
% % \small

% \centering
% \caption{The search results for the TFLite model in Android. We show the results of a fast way to identify the TFLite model in Android apps.  }
% \vspace{-0.5em}
% \begin{tabular}{l|cc}
% \toprule
%  \multicolumn{1}{c}{}  & Number of Apps & Number of TFLite Models \\
% \hline
% Results  & 674 & 262       \\

% % (0, 20)  & - & - & -     & -   & -      & -    &  - &  -       & -    & -  & \textbf{-}        \\
% \bottomrule
% \end{tabular}
% \label{tb:pre_model_file}
% \end{table}

\paragraph{\textbf{Results}}
We can easily find 674 apps using TensorFlow APIs (\eg \texttt{org.tensorflow}). 
After using the Apktool to unpack the App package~\footnote{\url{https://apktool.org/}}, we are eventually able to identify 262 TFLite models with 0\% of false positive identification rate. 
% The search steps just cost \textbf{less than 1 hour} using a Linux server with a workstation with Intel(R) Xeon(R) W-2175 2.50GHz CPU, and 32GB RAM. 
We conduct this experiment on 173,905 apps. However, Google Play store has 3.553 million apps until July 2023. Because the current deep learning technology has been proven to be vulnerable to various attack methods such as model invasion and model inversion attacks~\cite{huang2011adversarial}. All those apps using the DL models may have security issues if they can be easily identified by attackers. 

\begin{table}[t]
% \small
\centering
\caption{Statistics of apps with different numbers of TFLite models. The number of models in the most of apps is less than two. Note that apps usually have one kind of on-device model to save development costs and memory resources.}
\vspace{-0.5em}
\begin{tabular}{l|cccccc}
\hline
 Count of Models  & 1 & 2 & 3 & 4 & 5 & 6 \\
\hline
Count of Apps  & \ \ 109 \ \ & \ \ 86 \ \ & \ \ 18 \ \ & \ \ 16 \ \ & \ \ 21 \ \ & \ \ 12 \ \    \\

% (0, 20)  & - & - & -     & -   & -      & -    &  - &  -       & -    & -  & \textbf{-}        \\
\hline
\end{tabular}
\label{tb:pre_num_model}
\end{table}

\paragraph{\textbf{Analysis}}
As DL model files are easy to identify in real-world apps, we want to avoid using such model files in model deployment. Such DL model files are generated during the training period. Developers can easily save and load debuggable models for developing high-quality DL models. DL libraries and compilers like TFLite and TVM use rules to convert the computational representation of debuggable models to on-device representations. At the runtime, the DL library (\eg TFLite library) or TVM will load the computational graph and weights, then compute the data flow. In addition, we find most Apps need a limited number of models (\ie $\leq 2$), shown in Table~\ref{tb:pre_num_model}. Interaction between the model and library is not essential. We can fix the computational graph and weights in DL libraries of most AI programs to remove the model files. Thus, attackers cannot use keywords of model files to identify the DL components in apps.

\begin{tcolorbox}[colback=gray!5!white,colframe=gray!85]
As the model file will cause information leakage for deployed models, incorporating the computational graph and weights into a customized DL library program can help to reduce the exposure of DL components.
\end{tcolorbox}




% \subsection{Identifying Model Information}
% \label{sec:pre_info}
% In addition to locating model files, attackers can use specific in-model information to identify  DL components deployed on devices. In-model information contains the computational graph and tensor information. The computational graph is mainly composed of existing known DL operators (\eg `Conv2d' and `Softmax' in TFLite models). The operator information in TFLite models has the layer name, the spatial relationship with each other, and the index of inputs and weights. We can find the corresponding weights for each operator using the index.
% We investigate how to use keywords to identify such model information in model files.

% \begin{table}[t]
% % \begin{table}[t]
% % \footnotesize
% % \vspace{-1em}
%     \small
% 	\centering
%  \caption{Identification rate of in-model information using keywords. `Tensors': the tensor that should be allocated in the memory. `Operators': each neural layer. 
%  % The TVM model has two files: a graph file and a weights file. As the weights file just has numeric values of model weights, we omit it in our analysis. 
%  % However, as the TVM model files (\ie graph file and weights file) use low-level representations, It is hard to use specific keywords to identify the model information. 
%  }
%  \vspace{-0.5em}
% 	\begin{tabular}{l|c|c}
%  	\hline
%              \multicolumn{3}{c}{\bf Model Information in TFLite} \\
%              \hline
%          \makecell[c]{Example} & Number & Identification Rate\\
% 	 %  % \multicolumn{2}{*}{\bf Operator codes} \\
% 		% \hline
%   %       Original
%   %       &  "deprecated\_builtin\_code": 3 & 50 & \multirow{3}{*}{\bf 100\%} \\

%         % & $\cdots$ {\color{red} 4 codes in total} \\
%         % \cline{1-3}
%         % \multirow{2}{*}{Obfuscated}
%         % & "deprecated\_builtin\_code": 32, & \multirow{2}{*}{510} & \\
%         % & "custom\_code": "Fvsfxf", & & \\
%         % & "builtin\_code": "CUSTOM" & & \\

%         % &$\cdots$ {\color{red} 9 codes in total} \\
%         \hline
%              \multicolumn{3}{c}{Tensors} \\
%              % \hline
%         % &  \makecell[c]{Example} & Count & Ratio\\
% 		\hline
%         "shape": [1,224,224,3], & \multirow{5}{*}{1345} & \multirow{5}{*}{\bf 100\%} \\
%         "name": "conv2d\_1/Relu", & &\\

%         $\cdots$ & & \\
%         "shape": [500,3200], & &\\
%        "name": "dense\_1/kernel/transpose", & & \\
%         % &$\cdots$ {\color{red} 16 tensors in total} \\
%         % \cline{1-3}
%         % \multirow{2}{*}{Obfuscated}
%         % & "shape": [1,224,224,3], & \multirow{2}{*}{534} & \\
%         % & "name": "Fvsfxf", &  & \\

%         % &$\cdots$ {\color{red} 10 tensors in total}\\
%         \hline
%              \multicolumn{3}{c}{Operators} \\
% 	% \multicolumn{2}{c}{\bf Operators} & Count & Ratio \\
% 		\hline
%         "inputs": [3,2,0], & \multirow{4}{*}{510} & \multirow{4}{*}{\bf 100\%} \\
%         "outputs": [1], & & \\
%         "op\_type": "Conv2DOptions", & & \\
%         "builtin\_options": \{stride\_w: 1, $\cdots$\}, \ \ & & \\
%         % &$\cdots$ {\color{red} 7 operators in total} \\
%         % \cline{1-3}
%         % \multirow{4}{*}{Obfuscated} 
%         % & "inputs": [0], & \multirow{4}{*}{510} & \\
%         % & "outputs": [1], & & \\
%         % & "op\_type": "Fvsfxf", & & \\
%         % & "custom\_options": \{84,0,1,3,1, $\cdots$\}, & & \\

%         % &$\cdots$ {\color{red} 9 operators in total}\\
% 		\hline	
%         % \multicolumn{3}{c}{\bf Model Information in TVM} \\
%         % \hline
%         % \multicolumn{3}{c}{Low-level Representations} \\
%         % \hline
%         % `and eax, 0xfff' & \multirow{3}{*}{\XSolid} & \multirow{3}{*}{\XSolid} \\
%         % `cmp eax, 0x80' & & \\
%         % `jne 0x1068' & & \\
%         % \hline
% 	\end{tabular}
	

%  % \vspace{-2em}
%  \label{tb:pre_info}
% % \end{table}
% \end{table}

% \paragraph{\textbf{Study Process}}
% We collected 10 TFLite models including a fruit recognition model, a skin cancer diagnosis model, MobileNet~\citep{howard2017mobilenets}, MNASNet~\citep{tan2019mnasnet}, SqueezeNet~\citep{iandola2016squeezenet}, EfficientNet~\citep{tan2019efficientnet}, MiDaS~\citep{ranftl2020towards}, LeNet~\cite{lecun1998gradient}, PoseNet~\citep{kendall2015posenet}, and SSD~\citep{liu2016ssd}. 
% %We refer to them as model \ding{192} - \ding{201}, respectively. 
% The fruit recognition and skin cancer diagnosis model were collected from Android apps. The other models were collected from TensorFlow Hub~\footnote{\url{https://tfhub.dev/}}. 
% The TFLite model has two main kinds of information: `tensors' and `operators'. The `tensor' refers to the weights information of the model. The `operators' refers to the computational graph information. First, we extract the information of TFLite models into JSON files. Then, we use keywords of DL layers (\eg `\texttt{conv2d}') to search the corresponding DL layers in TFLite model files. After identifying the information in `operators', we can use the index of input and weights tensors (\eg "[3,2,0]" in the example) to find the corresponding weights information in `Tensors'. Results are shown in Table~\ref{tb:pre_info}. The potential keywords can be collected from the function names of the TensorFlow \texttt{tf.nn} module. We successfully identify all tensor and operator information in TFLite models via such keywords. It shows attackers can parse the model files and use such keywords to identify the DL components if the apps use TFLite models. 

% % \lili{no need to mention this. This is not helpful to motivate our work.}
% % However, after we convert the TFLite model to TVM models (\ie a graph file and a weights file), it is hard to use keywords to identify the DL components. This is because the low-level representation used in TVM does not have distinguishable keywords. 

% % \lili{following the same structure of Section 3.1: Study process -> result -> analysis}

% \paragraph{\textbf{Analysis}}
% % \lili{Same as my previous comment. This is not helpful for motivating our work.}
% % Low-level representations are effective to prevent attackers from identifying DL components on devices. We can refer to the AI compiler techniques to convert the high-level presentation to low-level representations of the computation graph to enhance the security of on-device DL models.
% The model information in the model file (\eg \texttt{.tflite} file) can be identified by the keyword search. Because standard DL libraries need to interact with the model file, the model file must be created in a specific format. DL library uses a rule list to parse the information in model files. Such a rule list can be collected by attackers as the DL libraries are usually open-sourced. For TVM, it has been proven that the model information in TVM can also be parsed and further reverse-engineered~\cite{chen2022learning}.

% \begin{tcolorbox}[colback=gray!5!white,colframe=gray!85]
% % Although model files compiled by AI compilers like TVM can be identified, the low-level representation can reduce the exposure of DL-related information.
% To enhance the model security, we can remove the model file in the deployment environment to prevent  extraction of inner information of DL models.
% \end{tcolorbox}

% %\subsection{Motivation for our Method}


==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*


.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

